FIRAL: An Active Learning Algorithm for Multinomial Logistic Regression

We investigate theory and algorithms for pool-based active learning for multiclass classification using multinomial logistic regression. Using finite sample analysis, we prove that the Fisher Information Ratio (FIR) lower and upper bounds the excess risk. Based on our theoretical analysis, we propose an active learning algorithm that employs regret minimization to minimize the FIR. To verify our derived excess risk bounds, we conduct experiments on synthetic datasets. Furthermore, we compare FIRAL with five other methods and found that our scheme outperforms them: it consistently produces the smallest classification error in the multiclass logistic regression setting, as demonstrated through experiments on MNIST, CIFAR-10, and 50-class ImageNet.

==> heavy-tailed.tex <==

%%%% assumptions
For heavy-tailed distribution, we have the following assumptions similar to the regularity assumptions in \cite{chaudhuri-2015}.
\begin{assumption}\label{assumption:heavy}
There exist constants $L_1, L_2$ and $L_3$, for any sample $(x,y)$ randomly drawn from distribution $\pi_p(x,y)$ or $\pi_q(x,y)$, the following conditions are satisfied: 
\begin{enumerate}[label={(\arabic*)},leftmargin=*]
\item concentration of gradient and Hessian around $\theta^*$: 
\begin{align}
     \| \mathrm{vec}(\nabla \ell_{(x,y)}(\theta^*) )\|_{\hp^{-1}} \leq L_1 ,\qquad
    \| \hp^{-1/2}\nabla^2 \ell_{(x,y)}(\theta^*)\hp^{-1/2} \| \leq L_2 ,\label{eq:heavy-assume-2}
\end{align}
\item Lipschitz continuity of Hessian: there exits a neighborhood around $\theta^*$ denoted by $B(\theta^*)$ such that $\forall \theta^\prime \in B(\theta^*)$, 
\begin{align}
    \Big\| \hp^{-1/2}\Big(\nabla^2 \ell_{(x,y)}(\theta^*) -  \nabla^2 \ell_{(x,y)}(\theta^\prime)\Big) \hp^{-1/2} \Big\| \leq L_3 \|\mathrm{vec}(\theta^* - \theta^\prime) \|_{\hp}.\label{eq:heavy-assume-3}
\end{align}
\end{enumerate}
\end{assumption}

%%============================
%%============================
%%%%% theorem: heavy-tailed distributions
%%============================
%%============================

\begin{theorem}\label{thm:heavy}
Suppose Assumption~\ref{assumption:heavy} holds. Define $\sigma:=\lambda_{\max}(\hq^{-1}\hp)$ for some constant $\sigma >1$.   For any $\delta \in (0,1)$, whenever 
\begin{align}\label{eq:heavy-n-bound}
    n \gtrsim \max \Big\{ L_2^2 \sigma^2 \log(2d(c-1)/\delta), \log(1/\delta) \sigma^4 L_1^2 L_3^2\Big\}
\end{align}
with probability at least $1-\delta$, we have 
\begin{align}\label{eq:heavy-risk-bound}
    \frac{3}{8} \frac{(1-\epsilon_p)}{(1+\epsilon_q)^2}  \frac{\Tr(\hq^{-1}\hp)}{n} &\leq \E [L_p(\emptheta)] - L_p(\theta^*)
    \leq \frac{5}{8} \frac{(1+\epsilon_p)}{(1-\epsilon_q)^2}  \frac{\Tr(\hq^{-1}\hp)}{n},
\end{align}
where $\E$ is the expectation over ${\{y_i\sim p(y_i|x_i, \theta^*)\}_{i=1}^n}$, $\epsilon_p$ and $\epsilon_q$ are given by
\begin{align}\label{eq:heavy-epsilon}
   \epsilon_p = 2 \sigma^2 L_1 L_3 \sqrt{\frac{2 + 8\log(1/\delta)}{n}}\, \quad\epsilon_q = 4 \sigma L_2 \sqrt{\frac{\log(2d(c-1)/\delta)}{n}} + 2 \sigma^2 L_1 L_3 \sqrt{\frac{2 + 8\log(1/\delta)}{n}}.
\end{align}
\end{theorem}

The proof details are given in Appendix~\ref{appendix:heavy-thm}. Similar to Theorem~\ref{thm:sub-thm}, $\frac{\Tr(\hq^{-1}\hp)}{n}$ is essential to excess risk since it shows up in both of the upper and lower bound (Equation~\eqref{eq:heavy-risk-bound}). Note that the coefficient of the upper bound $\frac{1+ \epsilon_p}{(1-\epsilon_q)^2}$ decreases as $\sigma$ decreases. Therefore, as $\Tr(\hq^{-1}\hp)$ decreases, we expect $\sigma$ also decreases, and the upper bound might converge faster than linear convergence rate. In addition,  under the premise of Theorem~\eqref{thm:heavy}, we show in our proof that $\epsilon_q \leq 3/8$ and $\epsilon_p \leq 1/8$, thus with probability at least $1-\delta$, we have $\E [L_p(\emptheta)] - L_p(\theta^*)
    \leq \frac{9}{5} \cdot \frac{\Tr(\hq^{-1}\hp)}{n}$.
    

